Word-Entity Duet Representations for Document Ranking

This paper presents a word-entity duet framework for utilizing knowledge bases in ad-hoc retrieval. In this work, the query and documents are modeled by word-based representations and entity-based representations. Ranking features are generated by the interactions between the two representations, incorporating information from the word space, the entity space, and the cross-space connections through the knowledge graph. To handle the uncertainties from the automatically constructed entity representations, an attention-based ranking model AttR-Duet is developed. With back-propagation from ranking labels, the model learns simultaneously how to demote noisy entities and how to rank documents with the word-entity duet. Evaluation results on TREC Web Track ad-hoc task demonstrate that all of the four-way interactions in the duet are useful, the attention mechanism successfully steers the model away from noisy entities, and together they significantly outperform both word-based and entity-based learning to rank systems.

==> table.tex <==

\begin{table*}[t]
\centering
\caption{Overall Performances of our methods comparing with baselines. 
% \texttt{ltr-duet} uses all four-way interaction ranking features in learning to rank without attention. 
\texttt{Att-LeToR-Duet} is the full model with duet ranking modules and attention mechanism.
Relative performances comparing with \texttt{RankSVM} are shown in percentages. \textbf{W}in/\textbf{T}ie/\textbf{L}oss are the number of queries a method improves, un-changes or hurts, compared with \texttt{RankSVM}. Best results in each metric are marked \textbf{Bold}. Statistic significant improvements ($p<0.05$) over \texttt{RankSVM}, \texttt{Coordinate Ascent}, \texttt{EQFE} and \texttt{EsdRank} are marked with $\dagger, \ddagger, \mathsection$, and $\mathparagraph$, respectively.
\label{tab:overall}
}

\begin{subtable}{1\textwidth}
\centering
\caption{ClueWeb09-B}
\begin{tabular}{l|lr|c|lr|c}
\hline
\bf{Method} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\bf{W/T/L} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L}
\\ \hline
\texttt{Lm}
 & ${0.1757}$ & $ -33.33\%  $

& 47/22/125

 & ${0.1195}$ & $ -22.63\%  $

& 49/22/123

\\
\texttt{SDM}
 & ${0.2496}$ & $ -5.26\%  $

& 62/32/100

 & ${0.1387}$ & $ -10.20\%  $

& 61/40/93

\\ \hline

\texttt{RankSVM}
 & $0.2635$ & --  & --/--/-- & $0.1544$ & --  & --/--/--\\
\texttt{Coordinate Ascent}
 & ${0.2681}$ & $ +1.75\%  $

& 71/41/82

 & ${0.1617}$ & $ +4.72\%  $

& 67/48/79

\\ \hline
\texttt{BOE-TagMe-Best}
 & ${0.2294}$ & $ -12.94\%  $

& 74/19/101

 & ${0.1488}$ & $ -3.63\%  $

& 72/20/102

\\
\texttt{EQFE}
 & ${0.2448}$ & $ -7.10\%  $

& 77/27/90

 & ${0.1419}$ & $ -8.10\%  $

& 80/29/85

\\
\texttt{EsdRank}
 & ${0.2644}$ & $ +0.33\%  $

& 88/22/84

 & ${0.1756}^{\mathsection }$ & $ +13.69\%  $

& 91/23/80

\\ \hline
\texttt{Att-LeToR-Duet}
 & ${0.3202}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +21.53\%  $

& 103/28/63

 & ${0.1985}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +28.55\%  $

& 100/32/62


\\
 \hline

\end{tabular}


\vspace*{1.5em}
\end{subtable}

\begin{subtable}{1\textwidth}
\centering
\caption{ClueWeb12-B13}
\begin{tabular}{l|lr|c|lr|c}
\hline
\bf{Method} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\bf{W/T/L} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L}
\\ \hline
\texttt{Lm}
 & ${0.1060}$ & $ -12.02\%  $

& 35/22/43

 & ${0.0863}$ & $ -6.67\%  $

& 38/21/41

\\
\texttt{SDM}
 & ${0.1083}$ & $ -10.14\%  $

& 27/25/48

 & ${0.0905}$ & $ -2.08\%  $

& 32/24/44

\\ \hline
\texttt{RankSVM}
 & $0.1205$ & --  & --/--/-- & $0.0924$ & --  & --/--/--\\
\texttt{Coordinate Ascent}
 & ${0.1206}$ & $ +0.08\%  $

& 36/32/32

 & ${0.0947}$ & $ +2.42\%  $

& 34/32/34

\\ \hline
\texttt{BOE-TagMe-Best}
 & ${0.1173}$ & $ -2.64\%  $

& 44/19/37

 & ${0.0950}$ & $ +2.83\%  $

& 43/19/38

\\ \hline
\texttt{Att-LeToR-Duet}
 & ${0.1351}^{\dagger \ddagger }$ & $ +12.14\%  $

& 44/25/31

 & ${0.1126}^{\dagger \ddagger }$ & $ +21.85\%  $

& 50/24/26



\\ \hline
\end{tabular}
\end{subtable}
\end{table*}




\begin{table*}[th]
\centering
\caption{Ranking Performance with each group of features from the word-entity duet.
\texttt{RankSVM} uses query's BOW and document's BOW. \texttt{LeToR-Qe-Dw} uses query's BOE and document's BOW, \texttt{LeToR-Qw-De} is query BOW + document BOE, and \texttt{LeToR-Qe-De} is query BOE + document BOE.
Relative performances comparing with corresponding base retrieval model are shown in percentages. \textbf{W}in/\textbf{T}ie/\textbf{L}oss are the number of queries a method improves, un-changes or hurts, compared with the base retrieval. 
% Best results in each metric are marked \textbf{Bold}. 
Statistic significant improvements ($p<0.05$) over the base retrieval are marked with $\dagger$.
\label{tab.ranking_res}
}

\begin{subtable}{1\textwidth}
\centering
\caption{ClueWeb09-B}
\begin{tabular}{l|lr|c|lr|c}
\hline
\bf{Method} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\bf{W/T/L} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L}
\\ \hline
\texttt{SDM}
 & $0.2496$ & --  & --/--/-- & $0.1387$ & --  & --/--/--\\
\texttt{RankSVM}
 & ${0.2635}^\dagger$ & $ +5.55\%  $

& 100/32/62

 & ${0.1544}^\dagger$ & $ +11.36\%  $

& 93/40/61

\\ \hline
\texttt{LeToR-Qe-Dw}
  & ${0.2729}$ & $ +9.33\%  $

& 82/28/84

 & ${0.1824}^\dagger$ & $ +31.51\%  $

& 86/29/79

\\
\texttt{LeToR-Qw-De}
 & ${0.2867}^\dagger$ & $ +14.83\%  $

& 91/33/70

 & ${0.1651}^\dagger$ & $ +19.07\%  $

& 88/35/71

\\
\texttt{LeToR-Qe-De}
 & ${0.2695}^\dagger$ & $ +7.97\%  $

& 99/34/61

 & ${0.1607}^\dagger$ & $ +15.88\%  $

& 95/42/57

\\ \hline
\end{tabular}
\end{subtable}

\vspace*{1.5em}

\begin{subtable}{1\textwidth}
\centering
\caption{ClueWeb12-B13}
\begin{tabular}{l|lr|c|lr|c}
\hline
\bf{Method} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\bf{W/T/L} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L}
\\ \hline
\texttt{Lm}
 & $0.1060$ & --  & --/--/-- & $0.0863$ & --  & --/--/--\\
\texttt{RankSVM}
 & ${0.1205}^\dagger$ & $ +13.67\%  $

& 43/22/35

 & ${0.0924}$ & $ +7.14\%  $

& 41/21/38

\\ \hline
\texttt{LeToR-Qe-Dw}
 & ${0.1110}$ & $ +4.66\%  $

& 40/20/40

 & ${0.0928}$ & $ +7.63\%  $

& 40/20/40


\\
\texttt{LeToR-Qw-De}
 & ${0.1146}$ & $ +8.09\%  $

& 42/20/38

 & ${0.0880}$ & $ +1.96\%  $

& 44/20/36

\\
\texttt{LeToR-Qe-De}
 & ${0.1166}$ & $ +10.01\%  $

& 38/20/42

 & ${0.0898}$ & $ +4.13\%  $

& 43/21/36

\\ \hline

\end{tabular}
\end{subtable}




\end{table*}


